Search for heavy resonances decaying into a $W$ or $Z$ boson and a Higgs boson in final states with leptons and $b$-jets in 36 fb$^{-1}$ of $\sqrt s = 13$ TeV $pp$ collisions with the ATLAS detector

A search is conducted for new resonances decaying into a $W$ or $Z$ boson and a 125 GeV Higgs boson in the $\nu\bar{\nu}b\bar{b}$, $\ell^{\pm}{\nu}b\bar{b}$, and $\ell^+\ell^-b\bar{b}$ final states, where $\ell^{\pm}= e^{\pm}$ or $\mu^{\pm}$, in $pp$ collisions at $\sqrt{s} = 13$ TeV. The data used correspond to a total integrated luminosity of 36.1 fb$^{-1}$ collected with the ATLAS detector at the Large Hadron Collider during the 2015 and 2016 data-taking periods. The search is conducted by examining the reconstructed invariant or transverse mass distributions of $Wh$ and $Zh$ candidates for evidence of a localised excess in the mass range of 220 GeV up to 5 TeV. No significant excess is observed and the results are interpreted in terms of constraints on the production cross-section times branching fraction of heavy $W^\prime$ and $Z^\prime$ resonances in heavy-vector-triplet models and the CP-odd scalar boson $A$ in two-Higgs-doublet models. Upper limits are placed at the 95% confidence level and range between $9.0\times 10^{-4}$ pb and $8.1\times 10^{-1}$ pb depending on the model and mass of the resonance.

==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2014-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATLAS-PUB-2014-XXX}
\AtlasNote{ATLAS-COM-PHYS-2014-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2014}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2014-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2014-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-PH-2014-XX}


==> sections/auxiliary.tex <==
\clearpage
\newpage
\input{sections/auxiliary_AZhPostfitCR}
\clearpage
\input{sections/auxiliary_pTV}
\clearpage
\input{sections/auxiliary_p0}
\clearpage
%\input{sections/auxiliary_bJetCorr}
%\clearpage
\input{sections/auxiliary_efficiency}
\clearpage


==> sections/auxiliary_AZhPostfitCR.tex <==
\begin{figure}[htb]
\centering
\subfloat[][ 2 lepton, 1+2 b-tag $e\mu$ CR]{
  \includegraphics[width=0.45\textwidth]{figures/postfit_bbA/incJet1_J2_T21_L2_distmVH_Dtopemucr_log}
}
\subfloat[][ 2 lepton, 3+ b-tag $e\mu$ CR]{
  \includegraphics[width=0.45\textwidth]{figures/postfit_bbA/incJet1_J2_incTag1_T3_L2_distmVH_Dtopemucr_log}
}
\caption{ 
Event distributions of  \MVh\ for the 2-lepton channel $e\mu$ control regions after a background-only fit to the categories used in the search for the $A$ boson produced in association with $b$-quarks.  
The quantity on the vertical axis is the number of data events divided by the bin width in \GeV.
The distribution for an $A$ boson with mass of 500~\GeV\  is shown as a red dashed line normalised using a cross-section of 5~pb.
The background uncertainty band shown includes both the statistical and systematic uncertainties after the fit added in quadrature. The lower panels show the ratio of the observed data to the estimated SM background.
}
\label{fig:mVH_AZhpostfit_3ptag}  
\end{figure}


==> sections/auxiliary_efficiency.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HVT 
\begin{figure}[tb]
\centering
\includegraphics[width=0.47\textwidth]{figures/efficiency_Zp_Zh_vvbb}
\includegraphics[width=0.47\textwidth]{figures/efficiency_Zp_Zh_llbb}
\\
\includegraphics[width=0.47\textwidth]{figures/efficiency_Wp_Wh_lvbb}
\caption{
Acceptance $\times$ reconstruction efficiency for the 
$Z^\prime\rightarrow Zh\rightarrow\nu\bar{\nu} b\bar{b}$ (top left),  
$Z^\prime\rightarrow Zh\rightarrow\ell^+\ell^- b\bar{b}$ (top right),  and
$W^\prime\rightarrow Wh\rightarrow\ell\nu b\bar{b}$ (bottom) 
processes in the signal regions defined in the text.  
} 
\label{fig:efficiency_HVT}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AZh 
\begin{figure}[tb]
\centering
\includegraphics[width=0.47\textwidth]{figures/efficiency_ggA_Zh_vvbb}
\includegraphics[width=0.47\textwidth]{figures/efficiency_ggA_Zh_llbb}
\\
\includegraphics[width=0.47\textwidth]{figures/efficiency_bbA_Zh_vvbb}
\includegraphics[width=0.47\textwidth]{figures/efficiency_bbA_Zh_llbb}
\caption{
Acceptance $\times$ reconstruction efficiency for the 
$A\rightarrow Zh \rightarrow\nu\bar{\nu} b\bar{b}$ (plots on the left) and
$A\rightarrow Zh \rightarrow\ell^+\ell^- b\bar{b}$ (plots on the right)
processes in the signal regions defined in the text.  
The plots on the top correspond to the gluon--gluon fusion production and 
the plots on the bottom to the $b$-quark associated production.
}
\label{fig:efficiencies_AZh}
\end{figure}


==> sections/auxiliary_efftables.tex <==
%%%%%%%%%%%%%%%%%Z'
{
\begin{table}[t]
\caption{\label{tab:EffTable_Zpvv} 
Acceptance * reconstruction efficiency for the $pp \rightarrow \Zprime \rightarrow Z\h \rightarrow \nu\nu\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c |  }
\hline\hline
%Mass 
%&  0-lep.,$\geq$ 2 jets, 1 $b$-tag
%&  0-lep.,$\geq$ 2 jets, 2 $b$-tag
%&  0-lep.,$\geq$ 1 large R jet, 1 $b$-tag 
%&  0-lep.,$\geq$ 1 large R jet, 2 $b$-tag

&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
\\
Mass 
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   1 $b$-tag 0 add $b$-tag
&   2 $b$-tag 0 add $b$-tag
\\ 
\hline \hline

500 & 0.0609877 & 0.120911 & 0.0010843 & 0.000291066\\
600 & 0.0889383 & 0.161682 & 0.0115274 & 0.00580863\\
700 & 0.115141 & 0.189919 & 0.0372978 & 0.019784\\
800 & 0.137557 & 0.205114 & 0.0536588 & 0.034184\\
900 & 0.157483 & 0.213514 & 0.062509 & 0.041993\\
1000 & 0.174177 & 0.21859 & 0.0716804 & 0.0486758\\
1100 & 0.189227 & 0.206071 & 0.0799805 & 0.0555581\\
1200 & 0.191208 & 0.184404 & 0.0981303 & 0.0716687\\
1300 & 0.177372 & 0.152974 & 0.124778 & 0.0972784\\
1400 & 0.155143 & 0.117336 & 0.156059 & 0.127754\\
1500 & 0.136985 & 0.0942966 & 0.184362 & 0.145547\\
1600 & 0.121848 & 0.0752833 & 0.207432 & 0.155853\\
1700 & 0.112091 & 0.0586128 & 0.226902 & 0.158544\\
1800 & 0.0959803 & 0.0510021 & 0.252386 & 0.158596\\
1900 & 0.0847492 & 0.0399345 & 0.273246 & 0.159698\\
2000 & 0.0778614 & 0.0338994 & 0.291183 & 0.157092\\
2200 & 0.0589428 & 0.0210863 & 0.313952 & 0.147465\\
2400 & 0.0505002 & 0.0161867 & 0.341523 & 0.129754\\
2600 & 0.0404438 & 0.0111486 & 0.358046 & 0.105298\\
2800 & 0.0339773 & 0.00797266 & 0.367537 & 0.0789625\\
3000 & 0.0263482 & 0.00624093 & 0.365175 & 0.0616516\\
3500 & 0.0153442 & 0.00280301 & 0.355518 & 0.0371056\\
4000 & 0.00791336 & 0.00147982 & 0.331134 & 0.0214428\\
4500 & 0.00552242 & 0.000552683 & 0.312535 & 0.0140142\\
5000 & 0.00321679 & 0.000268221 & 0.285142 & 0.0101984\\


\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}


%%%%%%%%%%%%%%%%%Z'
{
\begin{table}[t]
\caption{\label{tab:EffTable_Zpll} 
Acceptance * reconstruction efficiency for the $pp \rightarrow \Zprime \rightarrow Z\h \rightarrow \ell\ell\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c |  }
\hline\hline

&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
\\
Mass &  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   1 $b$-tag 0 add $b$-tag
&   2 $b$-tag 0 add $b$-tag
\\ 
\hline \hline

500 & 0.0681035 & 0.0972806 & 0.00128432 & 0.00032453\\
600 & 0.0840419 & 0.117132 & 0.00633158 & 0.00239691\\
700 & 0.0947861 & 0.129078 & 0.014937 & 0.00590359\\
800 & 0.109115 & 0.144487 & 0.0209028 & 0.0118786\\
900 & 0.12549 & 0.153337 & 0.0253629 & 0.0126833\\
1000 & 0.13532 & 0.151507 & 0.0289511 & 0.0172647\\
1100 & 0.140004 & 0.145633 & 0.0329673 & 0.021671\\
1200 & 0.138687 & 0.125042 & 0.0455387 & 0.0320751\\
1300 & 0.133953 & 0.102615 & 0.0650847 & 0.0539134\\
1400 & 0.11805 & 0.081057 & 0.0841969 & 0.0717741\\
1500 & 0.102307 & 0.0652699 & 0.103255 & 0.0878194\\
1600 & 0.093421 & 0.0524545 & 0.117944 & 0.0981615\\
1700 & 0.0803962 & 0.0418259 & 0.138565 & 0.101047\\
1800 & 0.0730833 & 0.034644 & 0.149447 & 0.101777\\
1900 & 0.0685335 & 0.0285622 & 0.161455 & 0.10436\\
2000 & 0.0596729 & 0.0234596 & 0.169176 & 0.0983314\\
2200 & 0.051476 & 0.0159935 & 0.185735 & 0.0927441\\
2400 & 0.0395478 & 0.0114888 & 0.200814 & 0.0802835\\
2600 & 0.0310189 & 0.00647548 & 0.213199 & 0.0626919\\
2800 & 0.0230591 & 0.00522991 & 0.210778 & 0.0463749\\
3000 & 0.0180942 & 0.00427801 & 0.20551 & 0.037437\\
3500 & 0.0102063 & 0.00164726 & 0.167402 & 0.0202372\\
4000 & 0.00583947 & 0.00079582 & 0.131372 & 0.0115315\\
4500 & 0.00376533 & 0.000621662 & 0.104502 & 0.00791682\\
5000 & 0.00300927 & 0.000284844 & 0.0886294 & 0.00531563\\

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}


%%%%%%%%%%%%%%%%%W'
{
\begin{table}[t]
\caption{\label{tab:EffTable_Wplv} 
Acceptance * reconstruction efficiency for the $pp \rightarrow \Wprime \rightarrow W\h \rightarrow \ell\nu\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c |  c |  c | c |  c | }
\hline\hline

&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  1-lep.
&  1-lep.
&  1-lep.
&  1-lep.

\\
Mass 
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   1 $b$-tag 
&   2 $b$-tag 
&   1 $b$-tag
&   2 $b$-tag
&   1 $b$-tag 
&   2 $b$-tag 
\\ 
&  
&   
&   0 add $b$-tag
&   0 add $b$-tag
&   
&   
&   0 add $b$-tag
&   0 add $b$-tag
\\ 
\hline \hline


500 & 0.00989954 & 0.018291 & 0.000182029 & 6.75549e-05 & 0.00989954 & 0.018291 & 0.000182029 & 6.75549e-05\\
600 & 0.015 & 0.0269261 & 0.00152722 & 0.00091265 & 0.015 & 0.0269261 & 0.00152722 & 0.00091265\\
700 & 0.0175684 & 0.0295484 & 0.00464995 & 0.00282662 & 0.0175684 & 0.0295484 & 0.00464995 & 0.00282662\\
800 & 0.0219954 & 0.0308973 & 0.00692232 & 0.00441198 & 0.0219954 & 0.0308973 & 0.00692232 & 0.00441198\\
900 & 0.0217527 & 0.0313719 & 0.00862834 & 0.00576719 & 0.0217527 & 0.0313719 & 0.00862834 & 0.00576719\\
1000 & 0.0219843 & 0.0315094 & 0.00990762 & 0.00547644 & 0.0219843 & 0.0315094 & 0.00990762 & 0.00547644\\
1100 & 0.0282306 & 0.0295536 & 0.00957134 & 0.00750316 & 0.0282306 & 0.0295536 & 0.00957134 & 0.00750316\\
1200 & 0.0263119 & 0.0259193 & 0.0118958 & 0.00840132 & 0.0263119 & 0.0259193 & 0.0118958 & 0.00840132\\
1300 & 0.0250362 & 0.0221221 & 0.0128702 & 0.0122238 & 0.0250362 & 0.0221221 & 0.0128702 & 0.0122238\\
1400 & 0.0195395 & 0.0164927 & 0.0183273 & 0.014849 & 0.0195395 & 0.0164927 & 0.0183273 & 0.014849\\
1500 & 0.0185582 & 0.0133276 & 0.0222606 & 0.0165335 & 0.0185582 & 0.0133276 & 0.0222606 & 0.0165335\\
1600 & 0.0162003 & 0.010178 & 0.0237842 & 0.0186268 & 0.0162003 & 0.010178 & 0.0237842 & 0.0186268\\
1700 & 0.0132365 & 0.00843588 & 0.0274786 & 0.0186879 & 0.0132365 & 0.00843588 & 0.0274786 & 0.0186879\\
1800 & 0.0133902 & 0.00645617 & 0.0324708 & 0.0180626 & 0.0133902 & 0.00645617 & 0.0324708 & 0.0180626\\
1900 & 0.0112721 & 0.00527523 & 0.0294729 & 0.0186141 & 0.0112721 & 0.00527523 & 0.0294729 & 0.0186141\\
2000 & 0.00931771 & 0.00510884 & 0.0337345 & 0.0171277 & 0.00931771 & 0.00510884 & 0.0337345 & 0.0171277\\
2200 & 0.00813947 & 0.00297425 & 0.0370391 & 0.0170487 & 0.00813947 & 0.00297425 & 0.0370391 & 0.0170487\\
2400 & 0.00629847 & 0.00232292 & 0.0383466 & 0.0147918 & 0.00629847 & 0.00232292 & 0.0383466 & 0.0147918\\
2600 & 0.00403833 & 0.00160515 & 0.039117 & 0.0102261 & 0.00403833 & 0.00160515 & 0.039117 & 0.0102261\\
2800 & 0.00451068 & 0.00104653 & 0.0431479 & 0.00740774 & 0.00451068 & 0.00104653 & 0.0431479 & 0.00740774\\
3000 & 0.00294805 & 0.000943825 & 0.0391369 & 0.00655661 & 0.00294805 & 0.000943825 & 0.0391369 & 0.00655661\\
3500 & 0.00192953 & 0.000314244 & 0.0375699 & 0.00349224 & 0.00192953 & 0.000314244 & 0.0375699 & 0.00349224\\
4000 & 0.000866316 & 0.00022722 & 0.0306292 & 0.00230869 & 0.000866316 & 0.00022722 & 0.0306292 & 0.00230869\\
4500 & 0.000681319 & 5.05565e-05 & 0.0297965 & 0.00149409 & 0.000681319 & 5.05565e-05 & 0.0297965 & 0.00149409\\
5000 & 0.000345248 & 7.11313e-05 & 0.0259772 & 0.000820506 & 0.000345248 & 7.11313e-05 & 0.0259772 & 0.000820506\\

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}






%%%%%%%%%%%%%%%%%ggAvv
{
\begin{table}[t]
\caption{\label{tab:EffTable_ggAvv} 
Acceptance * reconstruction efficiency for the $pp \rightarrow A \rightarrow Z\h \rightarrow \nu\nu\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c | c | c |  c |  }
\hline\hline
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
\\
Mass 
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   3+ $b$-tag
&   1 $b$-tag
&   2 $b$-tag
&   1 $b$-tag
&   2 $b$-tag
\\ 
&  
&  
&  
&    0 add $b$-tag
&    0 add $b$-tag
&    add $b$-tags
&    add $b$-tags
\\ 
\hline \hline

280 & 0.0009267 & 0.0002712 & 1.282e-05 & 2.28e-05 & 2.434e-06 & 7.128e-05 & 6.413e-06\\
300 & 0.001688 & 0.001274 & 5.425e-05 & 2.417e-05 & 0 & 0.0001193 & 7.996e-06\\
320 & 0.003273 & 0.003987 & 8.434e-05 & 3.143e-05 & 4.215e-06 & 0.0001492 & 7.045e-06\\
340 & 0.005634 & 0.009388 & 0.0002295 & 8.368e-05 & 1.572e-05 & 0.0002208 & 3.154e-05\\
360 & 0.009918 & 0.01832 & 0.0003297 & 0.0001775 & 6.644e-06 & 0.0003267 & 7.876e-06\\
380 & 0.01619 & 0.0322 & 0.0005587 & 0.0002375 & 1.207e-05 & 0.0004934 & 1.376e-05\\
400 & 0.02298 & 0.04829 & 0.0006052 & 0.0002913 & 2.77e-05 & 0.0004795 & 3.436e-05\\
420 & 0.02902 & 0.06213 & 0.0008964 & 0.0004947 & 4.035e-05 & 0.0005415 & 1.509e-05\\
440 & 0.03608 & 0.07586 & 0.001177 & 0.0006621 & 3.632e-05 & 0.0006072 & 5.128e-05\\
460 & 0.04085 & 0.08804 & 0.001388 & 0.0009469 & 5.241e-05 & 0.0006666 & 8.697e-05\\
480 & 0.04692 & 0.09736 & 0.001591 & 0.001102 & 0.0001444 & 0.0008317 & 7.042e-05\\
500 & 0.05003 & 0.1073 & 0.00165 & 0.001759 & 0.000257 & 0.0009282 & 7.792e-05\\
550 & 0.06079 & 0.1251 & 0.002119 & 0.005157 & 0.001625 & 0.001457 & 0.0002131\\
600 & 0.07115 & 0.1394 & 0.002408 & 0.01198 & 0.004977 & 0.001928 & 0.0004786\\
650 & 0.07883 & 0.1509 & 0.002773 & 0.02117 & 0.009745 & 0.002574 & 0.0006646\\
700 & 0.08566 & 0.1603 & 0.003114 & 0.03167 & 0.0159 & 0.003 & 0.001\\
750 & 0.09336 & 0.1688 & 0.003332 & 0.03896 & 0.02162 & 0.003671 & 0.001298\\
800 & 0.1005 & 0.1746 & 0.003746 & 0.04523 & 0.02617 & 0.003972 & 0.00152\\
850 & 0.1073 & 0.1794 & 0.00377 & 0.0517 & 0.03069 & 0.004297 & 0.001709\\
900 & 0.1137 & 0.183 & 0.004117 & 0.05502 & 0.03378 & 0.004416 & 0.001995\\
950 & 0.1213 & 0.1858 & 0.004132 & 0.05826 & 0.03674 & 0.004596 & 0.002096\\
1000 & 0.1264 & 0.1859 & 0.004126 & 0.06158 & 0.03993 & 0.004753 & 0.002252\\
1100 & 0.1361 & 0.1801 & 0.004311 & 0.07013 & 0.04627 & 0.005432 & 0.002814\\
1200 & 0.1393 & 0.167 & 0.003946 & 0.08165 & 0.05871 & 0.005528 & 0.003315\\
1300 & 0.1327 & 0.1442 & 0.003456 & 0.09805 & 0.07543 & 0.00616 & 0.003794\\
1400 & 0.1219 & 0.1223 & 0.003077 & 0.117 & 0.09346 & 0.00673 & 0.004266\\
1500 & 0.1126 & 0.1031 & 0.002513 & 0.1346 & 0.1042 & 0.007516 & 0.004926\\
1600 & 0.1037 & 0.08822 & 0.002261 & 0.1516 & 0.1136 & 0.007857 & 0.005201\\
1700 & 0.0952 & 0.07522 & 0.001827 & 0.1686 & 0.1187 & 0.00856 & 0.005294\\
1800 & 0.0883 & 0.06443 & 0.001489 & 0.1824 & 0.1211 & 0.008983 & 0.005467\\
1900 & 0.08085 & 0.05599 & 0.001295 & 0.196 & 0.1217 & 0.009638 & 0.005494\\
2000 & 0.0749 & 0.04849 & 0.001064 & 0.2085 & 0.1214 & 0.00983 & 0.005385\\

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}



%%%%%%%%%%%%%%%%%ggAll
{
\begin{table}[t]
\caption{\label{tab:EffTable_ggAll} 
Acceptance * reconstruction efficiency for the $pp \rightarrow A \rightarrow Z\h \rightarrow \ell\ell\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c | c | c |  }
\hline\hline
&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
\\
Mass 
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   3+ $b$-tag
&   1 $b$-tag
&   2 $b$-tag
&   1+2 $b$-tag
\\ 
& 
& 
& 
&  0 add $b$-tag
&  0 add $b$-tag
&  add $b$-tags
\\ 
\hline \hline

220 & 0.0294 & 0.04406 & 0.0005464 & 4.17e-05 & 6.269e-06 & 4.771e-05\\
240 & 0.04046 & 0.05908 & 0.0008153 & 5.654e-05 & 1.099e-05 & 8.581e-05\\
260 & 0.04516 & 0.06669 & 0.0008241 & 6.799e-05 & 1.177e-05 & 0.0001128\\
280 & 0.04869 & 0.07281 & 0.0009145 & 0.0001051 & 4.411e-05 & 0.000176\\
300 & 0.0515 & 0.07811 & 0.0009901 & 0.0002079 & 5.423e-05 & 0.0001562\\
320 & 0.05318 & 0.08222 & 0.001042 & 0.0002674 & 9.551e-05 & 0.0001786\\
340 & 0.05317 & 0.08381 & 0.001099 & 0.0004127 & 0.0001202 & 0.0002561\\
360 & 0.05416 & 0.08471 & 0.001079 & 0.0004478 & 0.0001446 & 0.0002861\\
380 & 0.05437 & 0.08582 & 0.001345 & 0.0005293 & 0.0001868 & 0.0003341\\
400 & 0.0546 & 0.08852 & 0.001333 & 0.0007523 & 0.0001657 & 0.0003505\\
420 & 0.056 & 0.09233 & 0.001382 & 0.0009383 & 0.0003068 & 0.0005249\\
440 & 0.05698 & 0.09389 & 0.001612 & 0.001263 & 0.000398 & 0.000599\\
460 & 0.05735 & 0.0968 & 0.001663 & 0.001616 & 0.000503 & 0.0006698\\
480 & 0.05956 & 0.1012 & 0.001602 & 0.002215 & 0.0006917 & 0.0007714\\
500 & 0.06107 & 0.1033 & 0.001684 & 0.002669 & 0.0008105 & 0.0008799\\
550 & 0.06407 & 0.1108 & 0.001955 & 0.005175 & 0.001767 & 0.001347\\
600 & 0.06886 & 0.1176 & 0.002043 & 0.008731 & 0.003311 & 0.001977\\
650 & 0.07359 & 0.124 & 0.002446 & 0.01322 & 0.004973 & 0.002505\\
700 & 0.07732 & 0.1285 & 0.002676 & 0.01712 & 0.007093 & 0.003157\\
750 & 0.08265 & 0.1338 & 0.00277 & 0.02029 & 0.008908 & 0.003637\\
800 & 0.0881 & 0.1383 & 0.002884 & 0.02361 & 0.01104 & 0.003945\\
850 & 0.09301 & 0.1417 & 0.003068 & 0.02597 & 0.01294 & 0.004375\\
900 & 0.09679 & 0.1428 & 0.00296 & 0.02837 & 0.01438 & 0.004689\\
950 & 0.1015 & 0.1427 & 0.003237 & 0.02971 & 0.01602 & 0.004985\\
1000 & 0.104 & 0.1418 & 0.003336 & 0.03232 & 0.01773 & 0.005412\\
1100 & 0.1107 & 0.1355 & 0.003235 & 0.03827 & 0.02384 & 0.006104\\
1200 & 0.1112 & 0.1233 & 0.003098 & 0.04835 & 0.03395 & 0.006834\\
1300 & 0.1064 & 0.1054 & 0.002547 & 0.06186 & 0.04924 & 0.00806\\
1400 & 0.09592 & 0.08883 & 0.002265 & 0.07709 & 0.06345 & 0.009317\\
1500 & 0.08874 & 0.07469 & 0.001968 & 0.09206 & 0.07252 & 0.01004\\
1600 & 0.08198 & 0.06315 & 0.001524 & 0.1046 & 0.08028 & 0.011\\
1700 & 0.07541 & 0.05311 & 0.001445 & 0.1163 & 0.08424 & 0.01165\\
1800 & 0.06958 & 0.04509 & 0.001173 & 0.128 & 0.08743 & 0.01194\\
1900 & 0.06364 & 0.03832 & 0.001086 & 0.1363 & 0.08771 & 0.01332\\
2000 & 0.05822 & 0.03311 & 0.0007513 & 0.1474 & 0.08814 & 0.01364\\

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}




%%%%%%%%%%%%%%%%%bbAvv
{
\begin{table}[t]
\caption{\label{tab:EffTable_bbAvv} 
Acceptance * reconstruction efficiency for the $pp \rightarrow bbA, A \rightarrow Z\h \rightarrow \nu\nu\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c | c | c |  c |  }
\hline\hline
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
&  0-lep.
\\
Mass 
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   3+ $b$-tag
&   1 $b$-tag
&   2 $b$-tag
&   1 $b$-tag
&   2 $b$-tag
\\ 
&  
&  
&  
&   0 add $b$-tag
&   0 add $b$-tag
&   add $b$-tags
&   add $b$-tags
\\ 

\hline \hline

280 & 0.0001401 & 0.0006067 & 1.577e-05 & 1.169e-05 & 0 & 6.842e-05 & 0\\
300 & 0.000609 & 0.0005241 & 0.0005949 & 0 & 0 & 0 & 4.202e-05\\
320 & 0.001104 & 0.002799 & 0.001268 & 6.711e-06 & 9.542e-06 & 0.0001597 & 2.882e-05\\
340 & 0.002328 & 0.005973 & 0.002477 & 3.28e-05 & 0 & 0.0002382 & 4.21e-05\\
360 & 0.005194 & 0.01249 & 0.004922 & 0 & 0 & 2.199e-05 & 0.0001035\\
380 & 0.009492 & 0.02283 & 0.008545 & 8.069e-05 & 0.0001076 & 0.0002306 & 1.821e-06\\
400 & 0.01613 & 0.03585 & 0.01164 & 0.0002296 & 0 & 0.0003206 & 5.047e-05\\
420 & 0.01909 & 0.0433 & 0.01598 & 0.0002606 & 2.696e-05 & 0.0004444 & 0.0001594\\
440 & 0.02397 & 0.0523 & 0.01939 & 0.0001142 & 9.223e-05 & 0.0004791 & 0.0001908\\
460 & 0.02869 & 0.06168 & 0.02169 & 0.0002345 & 0.0002141 & 0.0005239 & 0.0001856\\
480 & 0.03114 & 0.06936 & 0.02444 & 0.0003693 & 0.0002919 & 0.000824 & 0.0005117\\
500 & 0.03279 & 0.07546 & 0.02679 & 0.001042 & 0.0005512 & 0.002049 & 0.0004317\\
550 & 0.04337 & 0.08049 & 0.03233 & 0.002365 & 0.001177 & 0.004844 & 0.002105\\
600 & 0.04502 & 0.09113 & 0.03594 & 0.008862 & 0.00318 & 0.00819 & 0.005073\\
650 & 0.04936 & 0.09794 & 0.04356 & 0.01566 & 0.007563 & 0.01751 & 0.008138\\
700 & 0.05497 & 0.1037 & 0.04429 & 0.02383 & 0.01107 & 0.02196 & 0.01172\\
750 & 0.05779 & 0.1019 & 0.04684 & 0.0285 & 0.0169 & 0.02894 & 0.01603\\
800 & 0.06228 & 0.1062 & 0.05156 & 0.03275 & 0.01945 & 0.03717 & 0.01968\\
850 & 0.06586 & 0.1136 & 0.05257 & 0.03929 & 0.02204 & 0.03908 & 0.02155\\
900 & 0.07123 & 0.1082 & 0.0553 & 0.03717 & 0.02326 & 0.0406 & 0.02501\\
950 & 0.07074 & 0.1142 & 0.0525 & 0.04025 & 0.02313 & 0.04552 & 0.02644\\
1000 & 0.07647 & 0.1132 & 0.05904 & 0.0436 & 0.02809 & 0.04745 & 0.02878\\
1100 & 0.07928 & 0.1087 & 0.05794 & 0.04818 & 0.02926 & 0.05026 & 0.03318\\
1200 & 0.08095 & 0.09993 & 0.05063 & 0.04886 & 0.03259 & 0.05955 & 0.03791\\
1300 & 0.08092 & 0.08214 & 0.04241 & 0.06178 & 0.04291 & 0.06104 & 0.04375\\
1400 & 0.06768 & 0.07382 & 0.03531 & 0.06861 & 0.05573 & 0.07093 & 0.0481\\
1500 & 0.06415 & 0.06361 & 0.03052 & 0.08231 & 0.05786 & 0.07294 & 0.04932\\
1600 & 0.05843 & 0.05021 & 0.02276 & 0.09117 & 0.06371 & 0.07866 & 0.05263\\
1700 & 0.05646 & 0.04518 & 0.01996 & 0.09163 & 0.06608 & 0.0802 & 0.05603\\
1800 & 0.04754 & 0.03888 & 0.01698 & 0.1026 & 0.06973 & 0.08599 & 0.05499\\
1900 & 0.04308 & 0.03162 & 0.01542 & 0.1094 & 0.06746 & 0.09095 & 0.0532\\
2000 & 0.0425 & 0.02773 & 0.01122 & 0.1147 & 0.06721 & 0.0954 & 0.05309\\

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}



%%%%%%%%%%%%%%%%%bbAll
{
\begin{table}[t]
\caption{\label{tab:EffTable_bbAll} 
Acceptance * reconstruction efficiency for the $pp \rightarrow bbA, A \rightarrow Z\h \rightarrow \ell\ell\b\bar{b}$ process. 
}


\begin{center}
\begin{footnotesize}

\begin{tabular}{| l | c |  c | c |  c | c | c |  }
\hline\hline
&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
&  2-lep.
\\
Mass 
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$2 jets
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
&  $\geq$1 large-R jet
\\
&   1 $b$-tag
&   2 $b$-tag
&   3+ $b$-tag
&   1 $b$-tag
&   2 $b$-tag
&   1+2 $b$-tag
\\ 
&   
&   
&   
&    0 add $b$-tag
&    0 add $b$-tag
&    add $b$-tags
\\ 
\hline \hline

220 & 0.03085 & 0.04478 & 0.01375 & 0 & 0 & 0\\
240 & 0.03641 & 0.04841 & 0.01347 & 2.424e-05 & 2.236e-05 & 1.508e-06\\
260 & 0.03551 & 0.04956 & 0.01343 & 1.669e-05 & 0 & 5.739e-05\\
280 & 0.03818 & 0.05367 & 0.01643 & 0 & 1.663e-05 & -7.108e-05\\
300 & 0.04017 & 0.05918 & 0.01613 & 1.236e-05 & 7.642e-06 & 0.0002641\\
320 & 0.04118 & 0.06308 & 0.01764 & 1.182e-05 & 7.658e-07 & 0.0001592\\
340 & 0.04103 & 0.06271 & 0.01801 & 1.846e-05 & 4.707e-05 & 0.0002573\\
360 & 0.04161 & 0.06038 & 0.01699 & 0.0001303 & 5.479e-05 & 0.0003555\\
380 & 0.0409 & 0.06071 & 0.01948 & 0.0001041 & 1.519e-05 & 0.0003129\\
400 & 0.04039 & 0.06389 & 0.0185 & 0.0001697 & 4.745e-05 & 0.0004329\\
420 & 0.0392 & 0.06623 & 0.02018 & 0.0001986 & 0.0001123 & 0.0006963\\
440 & 0.03868 & 0.06318 & 0.02091 & 0.0003011 & 5.707e-05 & 0.0008345\\
460 & 0.04097 & 0.0659 & 0.02101 & 0.0001974 & 0.0001556 & 0.002041\\
480 & 0.04162 & 0.06444 & 0.02309 & 0.0006051 & 0.0004058 & 0.002415\\
500 & 0.0409 & 0.06733 & 0.02543 & 0.0003784 & 0.0004373 & 0.003665\\
550 & 0.04098 & 0.07134 & 0.02585 & 0.001605 & 0.0011 & 0.007191\\
600 & 0.04268 & 0.07052 & 0.03134 & 0.004632 & 0.002016 & 0.01076\\
650 & 0.04708 & 0.07494 & 0.03109 & 0.007136 & 0.00392 & 0.01929\\
700 & 0.04756 & 0.08013 & 0.03167 & 0.0104 & 0.00417 & 0.02603\\
750 & 0.04704 & 0.07685 & 0.03312 & 0.01391 & 0.006952 & 0.0313\\
800 & 0.051 & 0.0788 & 0.03857 & 0.01599 & 0.00727 & 0.03498\\
850 & 0.05543 & 0.08142 & 0.03879 & 0.01735 & 0.007812 & 0.04309\\
900 & 0.05817 & 0.07872 & 0.03966 & 0.01808 & 0.009067 & 0.04603\\
950 & 0.05873 & 0.0825 & 0.04231 & 0.01973 & 0.009504 & 0.05123\\
1000 & 0.06007 & 0.08421 & 0.04124 & 0.01909 & 0.009927 & 0.0565\\
1100 & 0.06275 & 0.07556 & 0.03876 & 0.02336 & 0.01168 & 0.062\\
1200 & 0.06209 & 0.07043 & 0.03565 & 0.02696 & 0.0172 & 0.06678\\
1300 & 0.05809 & 0.06128 & 0.0291 & 0.03185 & 0.02881 & 0.07732\\
1400 & 0.05194 & 0.0529 & 0.02308 & 0.04144 & 0.03456 & 0.08442\\
1500 & 0.04937 & 0.04463 & 0.01879 & 0.05213 & 0.03768 & 0.09458\\
1600 & 0.04337 & 0.03556 & 0.0147 & 0.05362 & 0.04115 & 0.1006\\
1700 & 0.04092 & 0.03456 & 0.01302 & 0.06007 & 0.04572 & 0.1042\\
1800 & 0.04012 & 0.02803 & 0.01098 & 0.06801 & 0.04507 & 0.1099\\
1900 & 0.03577 & 0.02718 & 0.009979 & 0.07134 & 0.04501 & 0.1083\\
2000 & 0.03305 & 0.02055 & 0.006814 & 0.07687 & 0.04801 & 0.1192\\

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}



==> sections/auxiliary_limittables.tex <==
%%%%%%%%%%%%%%%%%Z'
{
\begin{table}[t]
\caption{\label{tab:LimitTable_Zp} 
Observed and expected upper limits for the \Zprime\ search in pb.
}


\begin{center}

\begin{footnotesize}

\begin{tabular}{| l | c |   c | c |  c |  c | c | }
\hline\hline
Mass &  Observed & Expected - $2\sigma$ &  Expected - $1\sigma$ & Expected  & Expected + $1\sigma$ & Expected + $2\sigma$ \\ \hline \hline


500 & 0.129653 & 0.044691 & 0.059998 & 0.083267 & 0.116817 & 0.15929\\ \hline
600 & 0.022594 & 0.02098 & 0.028166 & 0.039089 & 0.054882 & 0.074924\\ \hline
700 & 0.014408 & 0.012377 & 0.016616 & 0.023059 & 0.032467 & 0.044545\\ \hline
800 & 0.008255 & 0.008173 & 0.010972 & 0.015227 & 0.021483 & 0.02957\\ \hline
900 & 0.012038 & 0.005624 & 0.00755 & 0.010478 & 0.014841 & 0.020551\\ \hline
1000 & 0.008396 & 0.004206 & 0.005646 & 0.007836 & 0.011162 & 0.015601\\ \hline
1100 & 0.005265 & 0.003581 & 0.004807 & 0.006672 & 0.009508 & 0.013296\\ \hline
1200 & 0.006098 & 0.003246 & 0.004358 & 0.006048 & 0.008636 & 0.012118\\ \hline
1300 & 0.004281 & 0.003104 & 0.004167 & 0.005783 & 0.008253 & 0.011575\\ \hline
1400 & 0.003192 & 0.002585 & 0.003471 & 0.004817 & 0.006907 & 0.009766\\ \hline
1500 & 0.00295 & 0.0023 & 0.003088 & 0.004285 & 0.006154 & 0.008717\\ \hline
1600 & 0.002307 & 0.001946 & 0.002613 & 0.003627 & 0.005246 & 0.007513\\ \hline
1700 & 0.001803 & 0.001575 & 0.002115 & 0.002935 & 0.004278 & 0.00623\\ \hline
1800 & 0.001657 & 0.001413 & 0.001897 & 0.002633 & 0.003846 & 0.005622\\ \hline
1900 & 0.001599 & 0.001251 & 0.00168 & 0.002332 & 0.003412 & 0.005006\\ \hline
2000 & 0.001582 & 0.001215 & 0.00163 & 0.002263 & 0.003311 & 0.004858\\ \hline
2200 & 0.001372 & 0.001045 & 0.001403 & 0.001947 & 0.002855 & 0.004266\\ \hline
2400 & 0.001193 & 0.000888 & 0.001192 & 0.001654 & 0.002437 & 0.003666\\ \hline
2600 & 0.00112 & 0.000806 & 0.001083 & 0.001503 & 0.002227 & 0.00336\\ \hline
2800 & 0.001077 & 0.000799 & 0.001073 & 0.001489 & 0.00221 & 0.003322\\ \hline
3000 & 0.00099 & 0.000791 & 0.001062 & 0.001473 & 0.002185 & 0.003279\\ \hline
3500 & 0.000897 & 0.000707 & 0.000949 & 0.001317 & 0.001976 & 0.003035\\ \hline
4000 & 0.00092 & 0.000684 & 0.000918 & 0.001274 & 0.00193 & 0.00304\\ \hline
4500 & 0.000927 & 0.000659 & 0.000885 & 0.001228 & 0.001862 & 0.003021\\ \hline
5000 & 0.00098 & 0.000669 & 0.000897 & 0.001246 & 0.001886 & 0.003142\\ \hline

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}


%%%%%%%%%%%%%%%%%W'
{
\begin{table}[t]
\caption{\label{tab:LimitTable_Wp} 
Observed and expected upper limits for the \Wprime\ search in pb.
}


\begin{center}

\begin{footnotesize}

\begin{tabular}{| l | c | c | c |  c |  c | c | }
\hline\hline
Mass &  Observed & Expected - $2\sigma$ &  Expected - $1\sigma$ & Expected  & Expected + $1\sigma$ & Expected + $2\sigma$ \\ \hline \hline

%500 & 0.28 & 0.11 & 0.15 & 0.21 & 0.30 & 0.40\\ \hline
%600 & 0.088 & 0.043 & 0.058 & 0.080 & 0.11 & 0.15\\ \hline
%700 & 0.045 & 0.021 & 0.028 & 0.039 & 0.054 & 0.074\\ \hline
%800 & 0.021& 0.011 & 0.015 & 0.021 & 0.030 & 0.041\\ \hline
%900 & 0.0010 & 0.0074 & 0.0099 & 0.014 & 0.019 & 0.027\\ \hline
%1000 & 0.0083 & 0.0051 & 0.0069 & 0.0094 & 0.014 & 0.019\\ \hline
%1100 & 0.0081 & 0.0042 & 0.0056 & 0.0078 & 0.011 & 0.016\\ \hline
%1200 & 0.0082 & 0.0036 & 0.0048 & 0.0068 & 0.0096 & 0.014\\ \hline
%1300 & 0.0071 & 0.0034 & 0.0045& 0.0063& 0.0090 & 0.013\\ \hline
%1400 & 0.0059 & 0.0034 & 0.0045 & 0.0063 & 0.0090 & 0.013\\ \hline
%1500 & 0.0049 & 0.0028 & 0.0037 & 0.0052 & 0.0074 & 0.010\\ \hline
%1600 & 0.0059 & 0.0024 & 0.0033 & 0.0045& 0.0065 & 0.0092\\ \hline
%1700 & 0.0051 & 0.0021 & 0.0029 & 0.0040 & 0.0057 & 0.0081\\ \hline
%1800 & 0.0027 & 0.0019 & 0.0025 & 0.0035 & 0.0050 & 0.0071\\ \hline
%1900 & 0.0018 & 0.0018 & 0.0024 & 0.0033 & 0.0048 & 0.0068\\ \hline
%2000 & 0.0015 & 0.0016 & 0.0022 & 0.0030 & 0.0044 & 0.0063\\ \hline
%2200 & 0.0011 & 0.0012 & 0.0016 & 0.0023 & 0.0033 & 0.0048\\ \hline
%2400 & 0.0018 & 0.0011 & 0.0014 & 0.0020 & 0.0029 & 0.0041\\ \hline
%2600 & 0.0020 & 0.00099 & 0.0013 & 0.0018 & 0.0027 & 0.0039\\ \hline
%2800 & 0.0021& 0.00094 & 0.0013 & 0.0017 & 0.0026 & 0.0037\\ \hline
%3000 & 0.0026 & 0.00086 & 0.0012 & 0.0016 & 0.0024 & 0.0035\\ \hline
%3500 & 0.0023 & 0.00078 & 0.0010 & 0.0014 & 0.0022 & 0.0033\\ \hline
%4000 & 0.0018 & 0.00075 & 0.0010& 0.0014 & 0.0021 & 0.0032\\ \hline
%4500 & 0.0014 & 0.00074 & 0.0010 & 0.0014 & 0.0021 & 0.0033\\ \hline
%5000 & 0.0013 & 0.00074 & 0.00099 & 0.0014 & 0.0021 & 0.0035\\ \hline

500 & 0.278603 & 0.114176 & 0.153282 & 0.212727 & 0.296223 & 0.399233\\ \hline
600 & 0.0882659 & 0.042993 & 0.0577182 & 0.0801024 & 0.111762 & 0.15108\\ \hline
700 & 0.0450127 & 0.0208442 & 0.0279834 & 0.0388359 & 0.0544033 & 0.0740339\\ \hline
800 & 0.0209823 & 0.0114609 & 0.0153863 & 0.0213535 & 0.0300058 & 0.0410296\\ \hline
900 & 0.00996169 & 0.00735916 & 0.00987968 & 0.0137112 & 0.0194488 & 0.0270026\\ \hline
1000 & 0.00826091 & 0.00514525 & 0.0069075 & 0.00958636 & 0.0136917 & 0.0192819\\ \hline
1100 & 0.00806434 & 0.00418472 & 0.00561799 & 0.00779675 & 0.0111498 & 0.0157378\\ \hline
1200 & 0.00819889 & 0.00358281 & 0.00480992 & 0.0066753 & 0.00961085 & 0.0137046\\ \hline
1300 & 0.00711971 & 0.00335627 & 0.0045058 & 0.00625324 & 0.00896864 & 0.0127423\\ \hline
1400 & 0.0059282 & 0.00338645 & 0.00454631 & 0.00630945 & 0.00896494 & 0.0125256\\ \hline
1500 & 0.00488335 & 0.00277093 & 0.00371998 & 0.00516266 & 0.00737325 & 0.0103769\\ \hline
1600 & 0.00594321 & 0.00243382 & 0.00326741 & 0.00453458 & 0.00649185 & 0.00916841\\ \hline
1700 & 0.00507633 & 0.00214299 & 0.00287697 & 0.00399272 & 0.00572785 & 0.00812488\\ \hline
1800 & 0.00268449 & 0.00188181 & 0.00252634 & 0.0035061 & 0.0050406 & 0.00717443\\ \hline
1900 & 0.0018061 & 0.00177527 & 0.0023833 & 0.00330759 & 0.00475723 & 0.00677349\\ \hline
2000 & 0.00152634 & 0.00161916 & 0.00217373 & 0.00301674 & 0.00436135 & 0.00625544\\ \hline
2200 & 0.00111521 & 0.00121347 & 0.00162909 & 0.00226088 & 0.00329243 & 0.00479777\\ \hline
2400 & 0.00179262 & 0.00105172 & 0.00141193 & 0.0019595 & 0.00285032 & 0.00414463\\ \hline
2600 & 0.00204356 & 0.000987725 & 0.00132602 & 0.00184028 & 0.00268128 & 0.00390251\\ \hline
2800 & 0.00206262 & 0.000938046 & 0.00125933 & 0.00174772 & 0.00255232 & 0.00372839\\ \hline
3000 & 0.00264128 & 0.000862443 & 0.00115783 & 0.00160686 & 0.00236299 & 0.00350121\\ \hline
3500 & 0.00229424 & 0.000777284 & 0.0010435 & 0.0014482 & 0.0021546 & 0.0032633\\ \hline
4000 & 0.00177004 & 0.000750981 & 0.00100819 & 0.00139919 & 0.00210319 & 0.0032463\\ \hline
4500 & 0.00143158 & 0.000737126 & 0.000989593 & 0.00137337 & 0.00208689 & 0.00334095\\ \hline
5000 & 0.00133078 & 0.000738598 & 0.000991569 & 0.00137612 & 0.00211164 & 0.00346556\\ \hline

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}



%%%%%%%%%%%%%%%%%HVT
{
\begin{table}[t]
\caption{\label{tab:LimitTable_HVT} 
Observed and expected upper limits for the HVT combined search with respect to the Model A predicted rate.
}


\begin{center}

\begin{footnotesize}

\begin{tabular}{| l | c |   c | c |  c |  c | c | }
\hline\hline
Mass &  Observed & Expected - $2\sigma$ &  Expected - $1\sigma$ & Expected  & Expected + $1\sigma$ & Expected + $2\sigma$ \\ \hline \hline

500 & 0.0447 & 0.0154 & 0.0207 & 0.0287 & 0.0402 & 0.0545\\ \hline
600 & 0.0188 & 0.0136 & 0.0183 & 0.0254 & 0.0355 & 0.0482\\ \hline
700 & 0.0214 & 0.0136 & 0.0182 & 0.0253 & 0.0355 & 0.0483\\ \hline
800 & 0.0168 & 0.0138 & 0.0185 & 0.0256 & 0.036 & 0.0492\\ \hline
900 & 0.022 & 0.0146 & 0.0196 & 0.0271 & 0.0383 & 0.0528\\ \hline
1000 & 0.0271 & 0.0158 & 0.0213 & 0.0295 & 0.0419 & 0.0583\\ \hline
1100 & 0.0333 & 0.0196 & 0.0263 & 0.0365 & 0.0519 & 0.0722\\ \hline
1200 & 0.0578 & 0.0248 & 0.0332 & 0.0461 & 0.0659 & 0.0926\\ \hline
1300 & 0.0647 & 0.0331 & 0.0444 & 0.0616 & 0.0879 & 0.1235\\ \hline
1400 & 0.0642 & 0.0442 & 0.0594 & 0.0824 & 0.1169 & 0.1626\\ \hline
1500 & 0.0763 & 0.0513 & 0.0689 & 0.0956 & 0.1361 & 0.1902\\ \hline
1600 & 0.1118 & 0.0596 & 0.0801 & 0.1111 & 0.1587 & 0.2232\\ \hline
1700 & 0.119 & 0.0679 & 0.0912 & 0.1265 & 0.1815 & 0.2574\\ \hline
1800 & 0.0944 & 0.0796 & 0.1068 & 0.1482 & 0.2131 & 0.3031\\ \hline
1900 & 0.0943 & 0.0965 & 0.1295 & 0.1798 & 0.2588 & 0.369\\ \hline
2000 & 0.1092 & 0.1175 & 0.1578 & 0.2189 & 0.3163 & 0.4531\\ \hline
2200 & 0.1381 & 0.1527 & 0.205 & 0.2845 & 0.4139 & 0.6024\\ \hline
2400 & 0.3391 & 0.2148 & 0.2884 & 0.4002 & 0.5819 & 0.8455\\ \hline
2600 & 0.6363 & 0.322 & 0.4323 & 0.5999 & 0.8729 & 1.2689\\ \hline
2800 & 0.9789 & 0.4949 & 0.6644 & 0.922 & 1.3433 & 1.9533\\ \hline
3000 & 1.9 & 0.7 & 1 & 1.3 & 2 & 2.9\\ \hline
3500 & 4.7 & 1.9 & 2.6 & 3.5 & 5.2 & 7.8\\ \hline
4000 & 10.1 & 5.2 & 6.9 & 9.6 & 14.3 & 21.9\\ \hline
4500 & 23.3 & 13.7 & 18.4 & 25.6 & 38.6 & 61.4\\ \hline
5000 & 62.4 & 38 & 51 & 70.8 & 107.9 & 176.4\\ \hline

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}


%%%%%%%%%%%%%%%%%ggA
{
\begin{table}[t]
\caption{\label{tab:LimitTable_ggA} 
Observed and expected upper limits for the $A$ search in gluon fusion production in pb.
}


\begin{center}

\begin{footnotesize}

\begin{tabular}{| l | c | c | c |  c |  c | c | }
\hline\hline
Mass &  Observed & Expected - $2\sigma$ &  Expected - $1\sigma$ & Expected  & Expected + $1\sigma$ & Expected + $2\sigma$ \\ \hline \hline

220 & 0.760899 & 0.543059 & 0.408394 & 0.54827 & 1.05895 & 1.4196\\ \hline
240 & 0.785126 & 0.807928 & 0.421398 & 0.565727 & 1.09267 & 1.4648\\ \hline
260 & 0.633011 & 0.672405 & 0.339753 & 0.45612 & 0.880969 & 1.181\\ \hline
280 & 0.562673 & 0.431714 & 0.302001 & 0.405437 & 0.783079 & 1.04977\\ \hline
300 & 0.419288 & 0.286503 & 0.225043 & 0.30212 & 0.583527 & 0.78226\\ \hline
320 & 0.332438 & 0.42477 & 0.178428 & 0.23954 & 0.462657 & 0.620225\\ \hline
340 & 0.26044 & 0.158343 & 0.139785 & 0.187662 & 0.362458 & 0.4859\\ \hline
360 & 0.221399 & 0.192906 & 0.11883 & 0.15953 & 0.308123 & 0.413061\\ \hline
380 & 0.167886 & 0.243432 & 0.0901086 & 0.120971 & 0.233648 & 0.313222\\ \hline
400 & 0.138881 & 0.22818 & 0.0745412 & 0.100072 & 0.193283 & 0.259109\\ \hline
420 & 0.114772 & 0.232623 & 0.0616013 & 0.0826999 & 0.15973 & 0.214129\\ \hline
440 & 0.095771 & 0.20968 & 0.0514028 & 0.0690083 & 0.133285 & 0.178679\\ \hline
460 & 0.0823757 & 0.132303 & 0.0442132 & 0.0593562 & 0.114643 & 0.153687\\ \hline
480 & 0.0704188 & 0.0814106 & 0.0377956 & 0.0507406 & 0.0980026 & 0.131379\\ \hline
500 & 0.0651388 & 0.111777 & 0.0349617 & 0.0469361 & 0.0906544 & 0.121529\\ \hline
550 & 0.0470694 & 0.0548937 & 0.0252634 & 0.0339161 & 0.065507 & 0.0878167\\ \hline
600 & 0.0377048 & 0.0191029 & 0.0202371 & 0.0271684 & 0.0524741 & 0.0703453\\ \hline
650 & 0.0281727 & 0.0187403 & 0.015121 & 0.0203 & 0.0392083 & 0.0525615\\ \hline
700 & 0.0228303 & 0.0143245 & 0.0122536 & 0.0164505 & 0.0317732 & 0.0425942\\ \hline
750 & 0.0203233 & 0.0130368 & 0.010908 & 0.0146441 & 0.0282841 & 0.0379169\\ \hline
800 & 0.0163821 & 0.00858329 & 0.00879269 & 0.0118042 & 0.0227991 & 0.0305638\\ \hline
850 & 0.0145147 & 0.00995274 & 0.00779041 & 0.0104586 & 0.0202003 & 0.0270799\\ \hline
900 & 0.011914 & 0.0118245 & 0.00639456 & 0.00858471 & 0.0165809 & 0.0222278\\ \hline
950 & 0.0110765 & 0.0129652 & 0.00594506 & 0.00798126 & 0.0154153 & 0.0206654\\ \hline
1000 & 0.00941356 & 0.0102848 & 0.0050525 & 0.00678299 & 0.013101 & 0.0175628\\ \hline
1100 & 0.00774439 & 0.00548329 & 0.00415661 & 0.00558026 & 0.0107779 & 0.0144486\\ \hline
1200 & 0.00691118 & 0.00779966 & 0.00370941 & 0.00497989 & 0.00961836 & 0.0128941\\ \hline
1300 & 0.00697831 & 0.00615908 & 0.00374544 & 0.00502826 & 0.00971179 & 0.0130193\\ \hline
1400 & 0.00627309 & 0.00487568 & 0.00336693 & 0.00452011 & 0.00873033 & 0.0117036\\ \hline
1500 & 0.00548749 & 0.00342878 & 0.00294528 & 0.00395404 & 0.007637 & 0.0102379\\ \hline
1600 & 0.00479023 & 0.00244605 & 0.00257104 & 0.00345163 & 0.00666662 & 0.00893708\\ \hline
1700 & 0.00415909 & 0.00213393 & 0.00223229 & 0.00299685 & 0.00578825 & 0.00775956\\ \hline
1800 & 0.00384627 & 0.00217185 & 0.00206439 & 0.00277145 & 0.0053529 & 0.00717593\\ \hline
1900 & 0.00373901 & 0.0020672 & 0.00200683 & 0.00269417 & 0.00520363 & 0.00697583\\ \hline
2000 & 0.00352106 & 0.00186863 & 0.00188984 & 0.00253712 & 0.0049003 & 0.0065692\\ \hline

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}


%%%%%%%%%%%%%%%%%bbA
{
\begin{table}[t]
\caption{\label{tab:LimitTable_bbA} 
Observed and expected upper limits for the $A$ search in $b$-quark associated production in pb. 
}


\begin{center}

\begin{footnotesize}

\begin{tabular}{| l | c |   c | c |  c |  c | c | }
\hline\hline
Mass &  Observed & Expected - $2\sigma$ &  Expected - $1\sigma$ & Expected  & Expected + $1\sigma$ & Expected + $2\sigma$ \\ \hline \hline

220 & 0.430216 & 0.3746 & 0.230908 & 0.309994 & 0.598736 & 0.802648\\ \hline
240 & 0.586021 & 0.730641 & 0.314532 & 0.42226 & 0.815571 & 1.09333\\ \hline
260 & 0.642615 & 0.604972 & 0.344908 & 0.463039 & 0.894334 & 1.19892\\ \hline
280 & 0.521051 & 0.385673 & 0.279662 & 0.375446 & 0.725153 & 0.972119\\ \hline
300 & 0.493907 & 0.271452 & 0.265093 & 0.355887 & 0.687375 & 0.921475\\ \hline
320 & 0.320332 & 0.25902 & 0.171931 & 0.230817 & 0.44581 & 0.59764\\ \hline
340 & 0.298324 & 0.161298 & 0.160118 & 0.214959 & 0.415181 & 0.556579\\ \hline
360 & 0.217515 & 0.153867 & 0.116746 & 0.156731 & 0.302718 & 0.405814\\ \hline
380 & 0.159649 & 0.162972 & 0.0856879 & 0.115036 & 0.222186 & 0.297856\\ \hline
400 & 0.155247 & 0.258098 & 0.0833248 & 0.111864 & 0.216058 & 0.289641\\ \hline
420 & 0.112088 & 0.283227 & 0.0601603 & 0.0807653 & 0.155994 & 0.20912\\ \hline
440 & 0.106129 & 0.289577 & 0.0569621 & 0.0764718 & 0.147701 & 0.198003\\ \hline
460 & 0.0899686 & 0.199457 & 0.0482885 & 0.0648274 & 0.12521 & 0.167853\\ \hline
480 & 0.0794992 & 0.129605 & 0.0426693 & 0.0572836 & 0.11064 & 0.148321\\ \hline
500 & 0.0717145 & 0.126958 & 0.038491 & 0.0516742 & 0.0998058 & 0.133797\\ \hline
550 & 0.0524059 & 0.0487894 & 0.0281276 & 0.0377613 & 0.0729338 & 0.0977729\\ \hline
600 & 0.0486388 & 0.0283099 & 0.0261057 & 0.035047 & 0.0676912 & 0.0907448\\ \hline
650 & 0.0342303 & 0.0287228 & 0.0183723 & 0.0246648 & 0.0476387 & 0.063863\\ \hline
700 & 0.0296781 & 0.0224608 & 0.015929 & 0.0213847 & 0.0413034 & 0.0553701\\ \hline
750 & 0.0274692 & 0.0188684 & 0.0147434 & 0.0197931 & 0.0382292 & 0.0512489\\ \hline
800 & 0.0211524 & 0.0117466 & 0.0113531 & 0.0152415 & 0.0294381 & 0.0394638\\ \hline
850 & 0.0184811 & 0.0120664 & 0.0099193 & 0.0133167 & 0.0257204 & 0.03448\\ \hline
900 & 0.0158061 & 0.0138738 & 0.00848356 & 0.0113892 & 0.0219976 & 0.0294893\\ \hline
950 & 0.0143104 & 0.0144952 & 0.00768078 & 0.0103115 & 0.019916 & 0.0266988\\ \hline
1000 & 0.0120665 & 0.0123484 & 0.00647638 & 0.00869456 & 0.016793 & 0.0225122\\ \hline
1100 & 0.0104017 & 0.00853456 & 0.00558287 & 0.00749501 & 0.0144762 & 0.0194063\\ \hline
1200 & 0.00980711 & 0.0112575 & 0.00526373 & 0.00706657 & 0.0136487 & 0.018297\\ \hline
1300 & 0.00939023 & 0.00906258 & 0.00503998 & 0.00676618 & 0.0130685 & 0.0175192\\ \hline
1400 & 0.00824497 & 0.00801244 & 0.00442529 & 0.00594096 & 0.0114746 & 0.0153825\\ \hline
1500 & 0.0068926 & 0.0057864 & 0.00369944 & 0.0049665 & 0.00959251 & 0.0128594\\ \hline
1600 & 0.00659282 & 0.00451774 & 0.00353854 & 0.00475049 & 0.0091753 & 0.0123001\\ \hline
1700 & 0.00548101 & 0.00347948 & 0.0029418 & 0.00394937 & 0.00762797 & 0.0102258\\ \hline
1800 & 0.00500067 & 0.00341194 & 0.00268399 & 0.00360326 & 0.00695948 & 0.00932968\\ \hline
1900 & 0.00514913 & 0.00383358 & 0.00276367 & 0.00371023 & 0.0071661 & 0.00960666\\ \hline
2000 & 0.00474158 & 0.0039301 & 0.00254493 & 0.00341657 & 0.00659891 & 0.0088463\\ \hline

\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}


==> sections/auxiliary_p0.tex <==
\begin{figure}[tb]
\centering
%\includegraphics[width=0.45\textwidth]{figures/limits/ggA_02_p0}
\includegraphics[width=0.45\textwidth]{figures/limits/bbA_02_p0}
\caption{
% The local p0 values for the combined fit for the $A$ boson assuming a pure gluon fusion (left) or $bbA$ production (right).
The observed probability (local p$_0$) that the background-only hypothesis would yield the same or more events in the combined fit for the $A$ boson in production with associated $b$-quarks. For  $m_A$ = 440 GeV, where the largest excess is observed, the local and global p$_0$ are quoted in the plot.
}
\label{fig:p0}
\end{figure}


==> sections/auxiliary_pTV.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HVT resolved (1,2 tag)
\begin{figure}[tb]
\centering
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/vvbb1tag2pjet_0ptv_SR_MET_fileOne__obs_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/vvbb2tag2pjet_0ptv_SR_MET_fileOne__obs_log}
\\
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/Ch1tag2pjet_0ptv_SR_pTV_fileTwo__obs_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/Ch2tag2pjet_0ptv_SR_pTV_fileTwo__obs_log}
\\
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/llbb1tag2pjet_0ptv_SR_pTV_fileThree__obs_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/llbb2tag2pjet_0ptv_SR_pTV_fileThree__obs_log}
\caption{
Event distributions of \met\  for the 0-lepton channel, \ptw\ for the 1-lepton channel,  and \ptll\ for the 2-lepton channel in the resolved categories.
The quantity on the vertical axis is the number of data events divided by the bin width in \GeV.
The background prediction is shown after a background-only maximum-likelihood fit to the data.
The signal for the benchmark HVT \textit{Model A} with $m_{V'} = 1.5 $~TeV is shown as a dashed red line and normalised to 10 times the theoretical cross-section.
The background uncertainty band shown includes both the statistical and systematic uncertainties after the fit added in quadrature. The lower panels show the ratio of the observed data to the estimated SM background.
} \label{fig:ptv_HVTpostfit_resolved}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HVT merged (1,2 tag)
\begin{figure}[tb]
\centering
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/vvbb1tag1pfat0pjet_0ptv_SR_noaddbjetsr_MET_fileOne__obs_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/vvbb2tag1pfat0pjet_0ptv_SR_noaddbjetsr_MET_fileOne__obs_log}
\\
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/Ch1tag1pfat0pjet_0ptv_SR_noaddbjetsr_pTV_fileTwo__obs_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/Ch2tag1pfat0pjet_0ptv_SR_noaddbjetsr_pTV_fileTwo__obs_log}
\\
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/llbb1tag1pfat0pjet_0ptv_SR_noaddbjetsr_pTV_fileThree__obs_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_HVT/llbb2tag1pfat0pjet_0ptv_SR_noaddbjetsr_pTV_fileThree__obs_log}
\caption{
Event distributions of \met\  for the 0-lepton channel, \ptw\ for the 1-lepton channel,  and \ptll\ for the 2-lepton channels in the merged categories.
The quantity on the vertical axis is the number of data events divided by the bin width in \GeV.
The background prediction is shown after a background-only  maximum-likelihood fit to the data.
The signal for the benchmark HVT \textit{Model A} with $m_{V'} = 1.5 $~TeV is shown as a dashed red line and normalised to 10 times the theoretical cross-section.
The background uncertainty band shown includes both the statistical and systematic uncertainties after the fit added in quadrature. The lower panels show the ratio of the observed data to the estimated SM background.
} \label{fig:ptv_HVTpostfit_merged}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AZh (3+tag)
\begin{figure}[tb]
\centering
\includegraphics[width=0.42\textwidth]{figures/postfit_bbA/incJet1_J2_incTag1_T3_L0_distMET_DSR_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_bbA/incJet1_J2_incTag1_T3_L2_distpTV_DSR_log}
\\
\includegraphics[width=0.42\textwidth]{figures/postfit_bbA/incFat1_Fat1_incJet1_J0_T1_L0_distMET_DSR_log}
\includegraphics[width=0.42\textwidth]{figures/postfit_bbA/incFat1_Fat1_incJet1_J0_T2_L0_distMET_DSR_log}
\\
\includegraphics[width=0.42\textwidth]{figures/postfit_bbA/incFat1_Fat1_incJet1_J0_T21_L2_distpTV_DSR_log}
\caption{
Event distributions of \met\  for the 0-lepton channel  and \ptll\ for the 2-lepton channel
after a background-only fit to the categories used in the search for the $A$ boson produced in association with $b$-quarks.  
The quantity on the vertical axis is the number of data events divided by the bin width in \GeV.
The distribution for an $A$ boson with mass of 500~\GeV\ (1.5\TeV) is shown as a red dashed line for illustration in the resolved (merged) regions normalised using a cross-section of 5~pb.
The background uncertainty band shown includes both the statistical and systematic uncertainties after the fit added in quadrature. The lower panels show the ratio of the observed data to the estimated SM background.
}
\label{fig:pTV_AZhpostfit}
\end{figure}

